TIDE: Time Derivative Diffusion for Deep Learning on Graphs

A prominent paradigm for graph neural networks is based on the message-passing framework. In this framework, information communication is realized only between neighboring nodes. The challenge of approaches that use this paradigm is to ensure efficient and accurate long-distance communication between nodes, as deep convolutional networks are prone to oversmoothing. In this paper, we present a novel method based on time derivative graph diffusion (TIDE) to overcome these structural limitations of the message-passing framework. Our approach allows for optimizing the spatial extent of diffusion across various tasks and network channels, thus enabling medium and long-distance communication efficiently. Furthermore, we show that our architecture design also enables local message-passing and thus inherits from the capabilities of local message-passing approaches. We show that on both widely used graph benchmarks and synthetic mesh and graph datasets, the proposed framework outperforms state-of-the-art methods by a significant margin

==> images/histogram.tex <==
\definecolor{plot1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{plot2}{rgb}{0.8500,0.3250,0.0980}
\definecolor{plot3}{rgb}{0.9290 0.6940 0.1250}

\begin{tikzpicture}%
%
\begin{axis}[
width=1.1\linewidth,
height=.9\linewidth,
grid=both,
grid style={line width=.1pt, draw=gray!50},
ybar = -2pt, 
bar width=2pt,
xmin=-0.05,
xmax=1.05, 
ymin=0,
xlabel={\small Value of time $t$},
ylabel={\small \% of total times},
y label style={at={(axis description cs:0.2,.5)},rotate=0,anchor=south},
x label style={at={(axis description cs:0.5,-0.1)},rotate=0,anchor=south},
xtick style={draw=none},
xtick =  {0,0.1,0.3,0.5,0.7,0.9},
%xticklabels = {0,1,2,3,4,5,6,7,8,9,10},
x tick label style = {font=\footnotesize, yshift=5pt},
y tick label style = {font=\footnotesize},
]%
%


\addplot[fill=plot1, draw=plot1] table[row sep=crcr]{%
0.98762584 0.015625  \\
0.89762896 0.0078125  \\
0.807632 0.0078125 \\
0.71763515 0.0234375  \\
0.6276383 0.1328125  \\
0.53764135 0.1953125  \\
0.44764447 0.28125  \\
0.35764757 0.21875  \\
0.2676507 0.09375  \\
0.17765379 0.0234375  \\
};


\end{axis}%
\end{tikzpicture}%
